Transverse-Momentum-Dependent Wave Functions of Pion from Lattice QCD

We present a first lattice QCD calculation of the transverse-momentum-dependent wave functions (TMDWFs) of the pion using large-momentum effective theory. Numerical simulations are based on one ensemble with 2+1+1 flavors of highly improved staggered quarks action with lattice spacing $a=0.121$~fm from the MILC Collaboration, and one with 2 +1 flavor clover fermions and tree-level Symanzik gauge action generated by the CLS Collaboration with $a=0.098$~fm. As a key ingredient, the soft function is first obtained by incorporating the one-loop perturbative contributions and a proper normalization. Based on this and the equal-time quasi-TMDWFs simulated on the lattice, we extract the light-cone TMDWFs. The results are comparable between the two lattice ensembles and a comparison with phenomenological parametrization is made. Our studies provide a first attempt of $ab$ $initio$ calculation of TMDWFs which will eventually lead to crucial theory inputs for making predictions for exclusive processes under QCD factorization.

==> main-references.tex <==
%\cite{Keum:2000wi}
\bibitem{Keum:2000wi}
Y.~Y.~Keum, H.~N.~Li and A.~I.~Sanda,
%``Penguin enhancement and $B \to K \pi$ decays in perturbative QCD,''
Phys. Rev. D \textbf{63}, 054008 (2001)
doi:10.1103/PhysRevD.63.054008
[arXiv:hep-ph/0004173 [hep-ph]].
%840 citations counted in INSPIRE as of 13 Jan 2023

%\cite{LHCb:2019hip}
\bibitem{LHCb:2019hip}
R.~Aaij \textit{et al.} [LHCb],
%``Search for lepton-universality violation in $B^+\to K^+\ell^+\ell^-$ decays,''
Phys. Rev. Lett. \textbf{122}, no.19, 191801 (2019)
doi:10.1103/PhysRevLett.122.191801
[arXiv:1903.09252 [hep-ex]].
%578 citations counted in INSPIRE as of 19 Jan 2023

%\cite{LHCb:2012de}
\bibitem{LHCb:2012de}
R.~Aaij \textit{et al.} [LHCb],
%``First observation of the decay $B^{+} \rightarrow \pi^{+} \mu^{+} \mu^{-}$,''
JHEP \textbf{12}, 125 (2012)
doi:10.1007/JHEP12(2012)125
[arXiv:1210.2645 [hep-ex]].
%101 citations counted in INSPIRE as of 11 Jan 2023

%\cite{Belle:2009zue}
\bibitem{Belle:2009zue}
J.~T.~Wei \textit{et al.} [Belle],
%``Measurement of the Differential Branching Fraction and Forward-Backward Asymmetry for $B \to K^{(*)}\ell^+\ell^-$,''
Phys. Rev. Lett. \textbf{103}, 171801 (2009)
doi:10.1103/PhysRevLett.103.171801
[arXiv:0904.0770 [hep-ex]].
%587 citations counted in INSPIRE as of 18 Jan 2023

%\cite{Brodsky:2001wx}
\bibitem{Brodsky:2001wx}
S.~J.~Brodsky,
%``QCD phenomenology and light front wavefunctions,''
Acta Phys. Polon. B \textbf{32}, 4013-4068 (2001)
[arXiv:hep-ph/0111340 [hep-ph]].
%34 citations counted in INSPIRE as of 29 Nov 2022

%\cite{Burkardt:2002uc}
\bibitem{Burkardt:2002uc}
M.~Burkardt, X.~d.~Ji and F.~Yuan,
%``Scale dependence of hadronic wave functions and parton densities,''
Phys. Lett. B \textbf{545}, 345-351 (2002)
doi:10.1016/S0370-2693(02)02596-0
[arXiv:hep-ph/0205272 [hep-ph]].
%34 citations counted in INSPIRE as of 09 Dec 2022

%\cite{Horn:2016rip}
\bibitem{Horn:2016rip}
T.~Horn and C.~D.~Roberts,
%``The pion: an enigma within the Standard Model,''
J. Phys. G \textbf{43}, no.7, 073001 (2016)
doi:10.1088/0954-3899/43/7/073001
[arXiv:1602.04016 [nucl-th]].
%135 citations counted in INSPIRE as of 20 Jan 2023

%\cite{Chang:2013pq}
\bibitem{Chang:2013pq}
L.~Chang, I.~C.~Cloet, J.~J.~Cobos-Martinez, C.~D.~Roberts, S.~M.~Schmidt and P.~C.~Tandy,
%``Imaging dynamical chiral symmetry breaking: pion wave function on the light front,''
Phys. Rev. Lett. \textbf{110}, no.13, 132001 (2013)
doi:10.1103/PhysRevLett.110.132001
[arXiv:1301.0324 [nucl-th]].
%215 citations counted in INSPIRE as of 20 Jan 2023

%\cite{LatticeParton:2022zqc}
\bibitem{LatticeParton:2022zqc}
J.~Hua \textit{et al.} [Lattice Parton],
%``Pion and Kaon Distribution Amplitudes from Lattice QCD,''
Phys. Rev. Lett. \textbf{129}, no.13, 132001 (2022)
doi:10.1103/PhysRevLett.129.132001
[arXiv:2201.09173 [hep-lat]].
%14 citations counted in INSPIRE as of 10 Jan 2023

%\cite{Cloet:2013tta}
\bibitem{Cloet:2013tta}
I.~C.~Clo\"et, L.~Chang, C.~D.~Roberts, S.~M.~Schmidt and P.~C.~Tandy,
%``Pion distribution amplitude from lattice-QCD,''
Phys. Rev. Lett. \textbf{111}, 092001 (2013)
doi:10.1103/PhysRevLett.111.092001
[arXiv:1306.2645 [nucl-th]].
%66 citations counted in INSPIRE as of 30 Nov 2022

%\cite{RQCD:2019osh}
\bibitem{RQCD:2019osh}
G.~S.~Bali \textit{et al.} [RQCD],
%``Light-cone distribution amplitudes of pseudoscalar mesons from lattice QCD,''
JHEP \textbf{08}, 065 (2019)
doi:10.1007/JHEP08(2019)065
[arXiv:1903.08038 [hep-lat]].
%72 citations counted in INSPIRE as of 05 Jan 2023

%\cite{Collins:2011ca}
\bibitem{Collins:2011ca}
J.~Collins,
%``New definition of TMD parton densities,''
Int. J. Mod. Phys. Conf. Ser. \textbf{4}, 85-96 (2011)
doi:10.1142/S2010194511001590
[arXiv:1107.4123 [hep-ph]].
%62 citations counted in INSPIRE as of 30 Dec 2022

%\cite{Collins:2014loa}
\bibitem{Collins:2014loa}
J.~Collins,
%``Different approaches to TMD Evolution with scale,''
EPJ Web Conf. \textbf{85}, 01002 (2015)
doi:10.1051/epjconf/20158501002
[arXiv:1409.5408 [hep-ph]].
%14 citations counted in INSPIRE as of 20 Nov 2022

%\cite{Keum:2000ph}
\bibitem{Keum:2000ph}
Y.~Y.~Keum, H.~n.~Li and A.~I.~Sanda,
%``Fat penguins and imaginary penguins in perturbative QCD,''
Phys. Lett. B \textbf{504}, 6-14 (2001)
doi:10.1016/S0370-2693(01)00247-7
[arXiv:hep-ph/0004004 [hep-ph]].
%732 citations counted in INSPIRE as of 08 Dec 2022

%\cite{Lu:2000em}
\bibitem{Lu:2000em}
C.~D.~Lu, K.~Ukai and M.~Z.~Yang,
%``Branching ratio and CP violation of B ---\ensuremath{>} pi pi decays in perturbative QCD approach,''
Phys. Rev. D \textbf{63}, 074009 (2001)
doi:10.1103/PhysRevD.63.074009
[arXiv:hep-ph/0004213 [hep-ph]].
%545 citations counted in INSPIRE as of 13 Jan 2023

%\cite{Lu:2007hr}
\bibitem{Lu:2007hr}
C.~D.~Lu, W.~Wang and Y.~M.~Wang,
%``Exclusive processes e+ e- ---\ensuremath{>} VP in k(T) factorization,''
Phys. Rev. D \textbf{75}, 094020 (2007)
doi:10.1103/PhysRevD.75.094020
[arXiv:hep-ph/0702085 [hep-ph]].
%20 citations counted in INSPIRE as of 01 Dec 2022

%\cite{Ali:2007ff}
\bibitem{Ali:2007ff}
A.~Ali, G.~Kramer, Y.~Li, C.~D.~Lu, Y.~L.~Shen, W.~Wang and Y.~M.~Wang,
%``Charmless non-leptonic $B_s$ decays to $PP$, $PV$ and $VV$ final states in the pQCD approach,''
Phys. Rev. D \textbf{76}, 074018 (2007)
doi:10.1103/PhysRevD.76.074018
[arXiv:hep-ph/0703162 [hep-ph]].
%310 citations counted in INSPIRE as of 23 Jan 2023

%\cite{Ji:2013dva}
\bibitem{Ji:2013dva}
X.~Ji,
%``Parton Physics on a Euclidean Lattice,''
Phys. Rev. Lett. \textbf{110}, 262002 (2013)
doi:10.1103/PhysRevLett.110.262002
[arXiv:1305.1539 [hep-ph]].
%565 citations counted in INSPIRE as of 20 Jan 2023

%\cite{Ji:2014hxa}
\bibitem{Ji:2014hxa}
X.~Ji, P.~Sun, X.~Xiong and F.~Yuan,
%``Soft factor subtraction and transverse momentum dependent parton distributions on the lattice,''
Phys. Rev. D \textbf{91}, 074009 (2015)
doi:10.1103/PhysRevD.91.074009
[arXiv:1405.7640 [hep-ph]].
%89 citations counted in INSPIRE as of 23 Dec 2022

%\cite{Ji:2020ect}
\bibitem{Ji:2020ect}
X.~Ji, Y.~S.~Liu, Y.~Liu, J.~H.~Zhang and Y.~Zhao,
%``Large-momentum effective theory,''
Rev. Mod. Phys. \textbf{93}, no.3, 035005 (2021)
doi:10.1103/RevModPhys.93.035005
[arXiv:2004.03543 [hep-ph]].
%160 citations counted in INSPIRE as of 20 Jan 2023

%\cite{Ji:2021znw}
\bibitem{Ji:2021znw}
X.~Ji and Y.~Liu,
%``Computing light-front wave functions without light-front quantization: A large-momentum effective theory approach,''
Phys. Rev. D \textbf{105}, no.7, 076014 (2022)
doi:10.1103/PhysRevD.105.076014
[arXiv:2106.05310 [hep-ph]].
%16 citations counted in INSPIRE as of 30 Nov 2022

%\cite{Li:2016ctv}
\bibitem{Li:2016ctv}
Y.~Li and H.~X.~Zhu,
%``Bootstrapping Rapidity Anomalous Dimensions for Transverse-Momentum Resummation,''
Phys. Rev. Lett. \textbf{118}, no.2, 022004 (2017)
doi:10.1103/PhysRevLett.118.022004
[arXiv:1604.01404 [hep-ph]].
%163 citations counted in INSPIRE as of 20 Jan 2023

%\cite{Ji:2019ewn}
\bibitem{Ji:2019ewn}
X.~Ji, Y.~Liu and Y.~S.~Liu,
%``Transverse-momentum-dependent parton distribution functions from large-momentum effective theory,''
Phys. Lett. B \textbf{811}, 135946 (2020)
doi:10.1016/j.physletb.2020.135946
[arXiv:1911.03840 [hep-ph]].
%54 citations counted in INSPIRE as of 20 Jan 2023

%\cite{Ji:2019sxk}
\bibitem{Ji:2019sxk}
X.~Ji, Y.~Liu and Y.~S.~Liu,
%``TMD soft function from large-momentum effective theory,''
Nucl. Phys. B \textbf{955}, 115054 (2020)
doi:10.1016/j.nuclphysb.2020.115054
[arXiv:1910.11415 [hep-ph]].
%53 citations counted in INSPIRE as of 20 Jan 2023

%\cite{LatticeParton:2020uhz}
\bibitem{LatticeParton:2020uhz}
Q.~A.~Zhang \textit{et al.} [Lattice Parton],
%``Lattice-QCD Calculations of TMD Soft Function Through Large-Momentum Effective Theory,''
Phys. Rev. Lett. \textbf{125}, no.19, 192001 (2020)
doi:10.22323/1.396.0477
[arXiv:2005.14572 [hep-lat]].
%62 citations counted in INSPIRE as of 20 Jan 2023

%\cite{Li:2021wvl}
\bibitem{Li:2021wvl}
Y.~Li, S.~C.~Xia, C.~Alexandrou, K.~Cichy, M.~Constantinou, X.~Feng, K.~Hadjiyiannakou, K.~Jansen, C.~Liu and A.~Scapellato, \textit{et al.}
%``Lattice QCD Study of Transverse-Momentum Dependent Soft Function,''
Phys. Rev. Lett. \textbf{128}, no.6, 062002 (2022)
doi:10.1103/PhysRevLett.128.062002
[arXiv:2106.13027 [hep-lat]].
%34 citations counted in INSPIRE as of 20 Jan 2023

%\cite{Shanahan:2021tst}
\bibitem{Shanahan:2021tst}
P.~Shanahan, M.~Wagman and Y.~Zhao,
%``Lattice QCD calculation of the Collins-Soper kernel from quasi-TMDPDFs,''
Phys. Rev. D \textbf{104}, no.11, 114502 (2021)
doi:10.1103/PhysRevD.104.114502
[arXiv:2107.11930 [hep-lat]].
%32 citations counted in INSPIRE as of 20 Jan 2023

%\cite{LPC:2022ibr}
\bibitem{LPC:2022ibr}
M.~H.~Chu \textit{et al.} [LPC],
%``Nonperturbative determination of the Collins-Soper kernel from quasitransverse-momentum-dependent wave functions,''
Phys. Rev. D \textbf{106}, no.3, 034509 (2022)
doi:10.1103/PhysRevD.106.034509
[arXiv:2204.00200 [hep-lat]].
%16 citations counted in INSPIRE as of 13 Jan 2023

%\cite{Schlemmer:2021aij}
\bibitem{Schlemmer:2021aij}
M.~Schlemmer, A.~Vladimirov, C.~Zimmermann, M.~Engelhardt and A.~Sch\"afer,
%``Determination of the Collins-Soper Kernel from Lattice QCD,''
JHEP \textbf{08}, 004 (2021)
doi:10.1007/JHEP08(2021)004
[arXiv:2103.16991 [hep-lat]].
%38 citations counted in INSPIRE as of 18 Jan 2023

%\cite{Deng:2022gzi}
\bibitem{Deng:2022gzi}
Z.~F.~Deng, W.~Wang and J.~Zeng,
%``Transverse-momentum-dependent wave functions and soft functions at one-loop in large momentum effective theory,''
JHEP \textbf{09}, 046 (2022)
doi:10.1007/JHEP09(2022)046
[arXiv:2207.07280 [hep-th]].
%2 citations counted in INSPIRE as of 29 Nov 2022

%\cite{Zhang:2022xuw}
\bibitem{Zhang:2022xuw}
K.~Zhang \textit{et al.} [[Lattice Parton Collaboration (LPC)]],
%``Renormalization of Transverse-Momentum-Dependent Parton Distribution on the Lattice,''
Phys. Rev. Lett. \textbf{129}, no.8, 082002 (2022)
doi:10.1103/PhysRevLett.129.082002
[arXiv:2205.13402 [hep-lat]].
%6 citations counted in INSPIRE as of 20 Jan 2023

\bibitem{supplemental}
Supplemental Material.

%\cite{Follana:2006rc}
\bibitem{Follana:2006rc}
E.~Follana \textit{et al.} [HPQCD and UKQCD],
%``Highly improved staggered quarks on the lattice, with applications to charm physics,''
Phys. Rev. D \textbf{75}, 054502 (2007)
doi:10.1103/PhysRevD.75.054502
[arXiv:hep-lat/0610092 [hep-lat]].
%595 citations counted in INSPIRE as of 23 Jan 2023

%\cite{MILC:2012znn}
\bibitem{MILC:2012znn}
A.~Bazavov \textit{et al.} [MILC],
%``Lattice QCD Ensembles with Four Flavors of Highly Improved Staggered Quarks,''
Phys. Rev. D \textbf{87}, no.5, 054505 (2013)
doi:10.1103/PhysRevD.87.054505
[arXiv:1212.4768 [hep-lat]].
%327 citations counted in INSPIRE as of 23 Jan 2023

%\cite{Hasenfratz:2001hp}
\bibitem{Hasenfratz:2001hp}
A.~Hasenfratz and F.~Knechtli,
%``Flavor symmetry and the static potential with hypercubic blocking,''
Phys. Rev. D \textbf{64}, 034504 (2001)
doi:10.1103/PhysRevD.64.034504
[arXiv:hep-lat/0103029 [hep-lat]].
%710 citations counted in INSPIRE as of 20 Jan 2023

%\cite{Ji:2020brr}
\bibitem{Ji:2020brr}
X.~Ji, Y.~Liu, A.~Sch\"afer, W.~Wang, Y.~B.~Yang, J.~H.~Zhang and Y.~Zhao,
%``A Hybrid Renormalization Scheme for Quasi Light-Front Correlations in Large-Momentum Effective Theory,''
Nucl. Phys. B \textbf{964}, 115311 (2021)
doi:10.1016/j.nuclphysb.2021.115311
[arXiv:2008.03886 [hep-ph]].
%51 citations counted in INSPIRE as of 20 Jan 2023

%\cite{Ebert:2019okf}
\bibitem{Ebert:2019okf}
M.~A.~Ebert, I.~W.~Stewart and Y.~Zhao,
%``Towards Quasi-Transverse Momentum Dependent PDFs Computable on the Lattice,''
JHEP \textbf{09}, 037 (2019)
doi:10.1007/JHEP09(2019)037
[arXiv:1901.03685 [hep-ph]].
%78 citations counted in INSPIRE as of 18 Jan 2023

%\cite{Ji:2017oey}
\bibitem{Ji:2017oey}
X.~Ji, J.~H.~Zhang and Y.~Zhao,
%``Renormalization in Large Momentum Effective Theory of Parton Physics,''
Phys. Rev. Lett. \textbf{120}, no.11, 112001 (2018)
doi:10.1103/PhysRevLett.120.112001
[arXiv:1706.08962 [hep-ph]].
%144 citations counted in INSPIRE as of 20 Jan 2023

%\cite{LatticePartonCollaborationLPC:2021xdx}
\bibitem{LatticePartonCollaborationLPC:2021xdx}
Y.~K.~Huo \textit{et al.} [Lattice Parton Collaboration (LPC)],
%``Self-renormalization of quasi-light-front correlators on the lattice,''
Nucl. Phys. B \textbf{969}, 115443 (2021)
doi:10.1016/j.nuclphysb.2021.115443
[arXiv:2103.02965 [hep-lat]].
%29 citations counted in INSPIRE as of 10 Jan 2023
